Transformer Inertial Poser: Real-time Human Motion Reconstruction from Sparse IMUs with Simultaneous Terrain Generation

Real-time human motion reconstruction from a sparse set of (e.g. six) wearable IMUs provides a non-intrusive and economic approach to motion capture. Without the ability to acquire position information directly from IMUs, recent works took data-driven approaches that utilize large human motion datasets to tackle this under-determined problem. Still, challenges remain such as temporal consistency, drifting of global and joint motions, and diverse coverage of motion types on various terrains. We propose a novel method to simultaneously estimate full-body motion and generate plausible visited terrain from only six IMU sensors in real-time. Our method incorporates 1. a conditional Transformer decoder model giving consistent predictions by explicitly reasoning prediction history, 2. a simple yet general learning target named "stationary body points" (SBPs) which can be stably predicted by the Transformer model and utilized by analytical routines to correct joint and global drifting, and 3. an algorithm to generate regularized terrain height maps from noisy SBP predictions which can in turn correct noisy global motion estimation. We evaluate our framework extensively on synthesized and real IMU data, and with real-time live demos, and show superior performance over strong baseline methods.

==> notes.tex <==
Real-time reconstruction of 3D human motion is crucial for applications in various domains, such as biomechanics and sports analysis, motion-based video games, and virtual presence in VR/AR systems. While marker-based optical motion capture systems~\cite{vicon} remain an ideal option for research labs and professional studios due to the superior accuracy, more and more applications demand a portable, less costly, and minimally-invasive mocap system that reconstructs human movements in real-time and can be used anywhere by everyone.

Among many proposed sensing modalities, such as RGB cameras \cite{}, depth cameras \cite{}, or wearable electromagnetic sensors [], inertial measurement sensors (IMUs) \cite{} have been singled out for many unique advantages they provide. IMU-based mocap is egocentric and untethered, applicable to both indoor and outdoor activities; is unsusceptible to occlusion; and is less sensitive to privacy issues. The state-of-the-art \cite{TransPose:SIG:2021} has shown that by learning multiple RNN models from large-scale human motion databases, such as AMASS~\cite{AMASS:ICCV:2019}, it is possible to estimate full 3D skeletal poses from only six IMUs.

This paper continues to push the state-of-the-art in real-time human motion reconstruction using six IMU sensors. Inspired by recent success of GPT-style models for natural language generation \cite{}, we propose a simple method based on a small GPT model which takes as input XXX and predicts XXX. Comparing to the state-of-the-art, our model improved human motion reconstruction both qualitatively and qualitatively across a large variety of motion types. In particular, previous RNN-based models do not explicitly make use of its own previous predictions, and thus struggle to distinguish between motion trajectories with similar orientations and persistent zero-acceleration, such as sitting versus standing \cite{}. As GPT models condition on the entire history of past predictions when making next prediction, our method could create consistent long sitting motion without switching between sitting and standing poses.

Another fundamental challenge in IMU-based system is the reconstruction of the root motion in which small errors usually accumulate rapidly due to the lack of feedback correction. Previous motion modeling algorithms\cite{} rely on heuristics to detect or learn the current supporting foot and enforce the foot to be stationary. This method tends to generate "foot locking" artifacts and fail to handle non-locomotion or locomotion over non-flat terrains (e.g. slope, stairs). In this work, we found that devising such engineering solutions is unnecessary. Instead, if we simply add an auxiliary task to predict "stationary body points" (\ie a Cartesian point on the character that has zero velocity) from the previous time step during training, the GPT model learns to predict the root motion with higher accuracy. Furthermore, we could use the predicted stationary points during test time to correct the predicted pose. This is particularly helpful when the distribution of the testing set is significantly different from that of the training set due to noisy or corrupted IMU sensors, or unseen motion.

Our new algorithm achieves new state-of-the-art results on both synthesized and real IMU reconstruction datasets. In practice, our model is easy to implement and smaller in size therefore faster to inference, compared to existing methods. We also evaluate our method on... (depending on what experiments we have time to finish)

